Resonant Dynamics and the Instability of the Box Minkowski Model

We revisit the box Minkowski model [Phys. Rev. Lett. 109, 221101 (2012)] and provide a strong argument that, subject to the Dirichlet boundary condition, it is unstable toward black hole formation for arbitrarily small generic perturbations. Using weakly nonlinear perturbation theory, we derive the resonant system, which compared to systems with the anti-de Sitter asymptotics, has extra resonant terms, and study its properties, including conserved quantities. We find that the generic solution of the resonant system becomes singular in finite time. Surprisingly, the additional resonant interactions do not significantly affect the singular evolution. Furthermore, we find that the interaction coefficients take a relatively simple form, making this a particularly attractive toy model of turbulent gravitational instability.

==> macros.tex <==
% File: macros.tex
% Description:
% Version: 0.1.0
% Author: Maciej Maliborski, maciej.maliborski@gmail.com

\usepackage[dvipsnames]{xcolor}
\usepackage{soul}
\usepackage[colorinlistoftodos, textwidth=1.75cm]{todonotes}
%% https://ctan.org/pkg/showkeys
%% options: final, draft
\usepackage[color, final]{showkeys}
\reversemarginpar
\usepackage[normalem]{ulem} % For \xout; normalem option fixes the issue with underline in bibliography (see https://stackoverflow.com/questions/51132189)

\setlength{\marginparwidth}{1.75cm}

% Miniscule font size (smaller than tiny)
\usepackage{lmodern}
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother

% Margin comment sizes
\def\margincomentfontsize{\tiny}
\newcounter{todocounter}
\newcommand{\todonum}[2][]{
        \stepcounter{todocounter}\todo[#1]{\thetodocounter: #2}
}


%% The showkeys package settings
% Colors
\definecolor{refkey}{gray}{.75}
\definecolor{labelkey}{gray}{.55}
% Font size and font family
\renewcommand*{\showkeyslabelformat}[1]{\fbox{\ttfamily\tiny{#1}}}


% Math definitions
%% Math symbols
\def\diff{\mathrm{d}}
\def\ep{\varepsilon}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\diag}{diag}
\def\transpose{\intercal}
% \renewcommand*{\i}{\imath}
\def\i{\mathrm{i}} % Complex I
\def\1{\mathbb{1}} % Bold 1
\def\id{\1} % Identity matrix/operator; same as bold 1
\def\idop{\mathrm{id}}
\def\R{\mathbb{R}}
\def\eth{{\text\dh}}
\def\ethb{\bar{{\text\dh}}}
%% Math commands
\newcommand{\define}[1]{\textit{#1}}
\newcommand{\doverd}[1]{\frac{\diff}{\diff{#1}}}
\newcommand{\pdoverpd}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\code}[1]{{\tt\detokenize{#1}}}
\newcommand{\der}[2]{\frac{\diff #1}{\diff #2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\psbr}[2]{\left\{#1,#2\right\}}
\newcommand{\bigO}[1]{\mathcal{O}\left({#1}\right)}
%% Theorems
\newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
% \newtheorem{exercise}{Exercise}



% The following requires todonotes, soul and color/xcolor packages
\makeatletter
\if@todonotes@disabled
\newcommand{\error}[1]{}
\newcommand{\warning}[1]{}
\newcommand{\comment}[1]{}
\newcommand{\fixthis}[2]{#1}
\else
\newcommand{\fixthis}[2]{\texthl{#1}\warning{#2}}
\newcommand{\error}[1]{\todonum[color=RedOrange,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\warning}[1]{\todonum[tickmarkheight=0.5ex, color=TealBlue,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\comment}[1]{\todonum[color=Goldenrod,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\checkedon}[1]{\todo[color=Gray!20!White, size=\margincomentfontsize]{\ttfamily{Checked on: #1}}}
%
\newcommand{\notecom}[1]{\todonum[color=Goldenrod,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\noteref}[1]{\todonum[color=YellowGreen,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\noteimp}[1]{\todonum[color=RedOrange,size=\margincomentfontsize]{\ttfamily{#1}}}
%
\fi
\makeatother


% Edit commands
\newcommand{\editremove}[1]{}
\newcommand{\edittrash}[1]{}
%% Highlight
\newcommand{\edithigh}[1]{\texthl{#1}}
\newcommand{\editcross}[1]{\xout{#1}}
\newcommand{\editreplace}[2]{\editcross{#1}\edithigh{#2}}
%\def\lightblue{\color{Cyan!50!White}}
\colorlet{lightblue}{Cyan!40!White}
\newcommand{\editadd}[1]{{\sethlcolor{lightblue}\texthl{#1}}}
\colorlet{lightpink}{Magenta!50!White}
\newcommand{\editimp}[1]{{\sethlcolor{lightpink}\texthl{#1}}}
\colorlet{lightorange}{Orange!60!White}
\newcommand{\editword}[1]{{\sethlcolor{lightorange}\texthl{#1}}}


%% Color font
\newcommand{\editinred}[1]{{\color{red} #1}}
\newcommand{\editinblue}[1]{{\color{blue} #1}}
%% Notes
\newcommand{\editnotecom}[1]{\todonum[color=Goldenrod,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\editnoteref}[1]{\todonum[color=YellowGreen,size=\margincomentfontsize]{\ttfamily{#1}}}
\newcommand{\editnoteimp}[1]{\todonum[color=RedOrange,size=\margincomentfontsize]{\ttfamily{#1}}}


%%% Final
%\renewcommand{\editreplace}[2]{#2}
%\renewcommand{\editcross}[1]{}
%\renewcommand{\edithigh}[1]{#1}
%\renewcommand{\editadd}[1]{#1}
%\renewcommand{\editimp}[1]{#1}

